Counterfactual Graph Augmentation for Consumer Unfairness Mitigation in Recommender Systems

In recommendation literature, explainability and fairness are becoming two prominent perspectives to consider. However, prior works have mostly addressed them separately, for instance by explaining to consumers why a certain item was recommended or mitigating disparate impacts in recommendation utility. None of them has leveraged explainability techniques to inform unfairness mitigation. In this paper, we propose an approach that relies on counterfactual explanations to augment the set of user-item interactions, such that using them while inferring recommendations leads to fairer outcomes. Modeling user-item interactions as a bipartite graph, our approach augments the latter by identifying new user-item edges that not only can explain the original unfairness by design, but can also mitigate it. Experiments on two public data sets show that our approach effectively leads to a better trade-off between fairness and recommendation utility compared with state-of-the-art mitigation procedures. We further analyze the characteristics of added edges to highlight key unfairness patterns. Source code available at https://github.com/jackmedda/RS-BGExplainer/tree/cikm2023.

==> review.tex <==
1) Motivation not clearly presented (why counterfactual explanations are relevant and how they can be used to mitigate unfairness in recommender systems, or how they can address the limitations of existing approaches.)
2) Lacking theoretical support (Counterfactual is a concept from the causal theory, and causal analysis is necessary for discussing counterfactual explanations. The authors should provide more theoretical insights into the working principles of their approach.) => eviedenziare che noi trattiamo le azioni degli utenti come aspetti che possano giustamente influenzare le raccomandazioni (poiché il modello impara da esse) e quindi anche la fairness. In particolare il modello è stato maggiormente influenzato dalle azioni del gruppo avvantaggiato, quindi se ipotizzassimo (in un mondo counteractual) che il gruppo svantaggiato avesse fatto più azioni, allora il modello potrebbe subite un impatto positivo da queste azioni, senza danneggiare l'esperienza degli utenti avvantaggiati.
3) Discussion in Table 1
4) Missing highlighting of explainability in motivation. How we are leveraging explainability in Eq. (3)? => Use Explainable Fairness => if fairness if mitigated, the applied change can be used as explanation
5) It is unclear how the loss mitigates unfairness => highlight that we augment the interactions of the disadvantaged group to boost their recommendations utility
6) clearer explanations of the methodology (graph augmentation process, perturbation mechanism) Some details and equations are not well-explained.
7) The paper lacks a detailed discussion of the limitations and potential drawbacks of the proposed approach.

----------------------------------------------------------------
----------------------------------------------------------------
----------------------------------------------------------------

SUBMISSION: 2376
TITLE: Counterfactual Graph Augmentation for Consumer Unfairness Mitigation in Recommender Systems

-------------------------  METAREVIEW  ------------------------
The authors address consumer unfairness in recommendation systems and propose leveraging counterfactual explanations to mitigate it. Extensive experiments demonstrate the effectiveness of the proposed method. However, the motivation is not clearly presented, and the method lacks sufficient theoretical support. More discussions should also be included to analyze the performance.



----------------------- REVIEW 1 ---------------------
SUBMISSION: 2376
TITLE: Counterfactual Graph Augmentation for Consumer Unfairness Mitigation in Recommender Systems
AUTHORS: Giacomo Medda, Francesco Fabbri, Mirko Marras, Ludovico Boratto and Gianni Fenu

----------- Strengths -----------
The paper nicely motivates the need of the proposed work in the Introduction.

Decent solution, nicely presented, even if some motivation decisions are missing. But still it is ok, given the pages limit.
----------- Weaknesses -----------
The datasets used are well-known and with relevant sensitive attributes. However it will be nice to exploit other datasets that include additional sensitive attributes. In these set of experiments, both datasets have the same sensitive attributes.
----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
For a survey on fairness in recommender systems, please cite:
E. Pitoura et al. Fairness in Rankings and Recommendations: An Overview. The VLDB Journal, 2022



----------------------- REVIEW 2 ---------------------
SUBMISSION: 2376
TITLE: Counterfactual Graph Augmentation for Consumer Unfairness Mitigation in Recommender Systems
AUTHORS: Giacomo Medda, Francesco Fabbri, Mirko Marras, Ludovico Boratto and Gianni Fenu

----------- Strengths -----------
1. Unfairness and explainability are hot topics in recommendation systems.
2. The paper is well-structured and concise.
3. They open their codebase.
----------- Weaknesses -----------
1. The problem formulation is unclear. Explainability is not included in the formulation although the introduction and abstract emphasize explainability.
2. It is unclear why the method can reduce unfairness.
3. The evaluations of unfairness are hard to understand (i.e., Table 1)
----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
This paper tackles the fairness problem of recommendation systems. This paper is well-structured and is easy to read generally. However, this paper has an inconsistency: in the abstract and introduction, they emphasize the importance to combine fairness and explainability, while the problem formulation does not include any explainability. Also, it is unsure why their method can reduce the unfairness: it seems just caused by loss function (i.e., Eq (3)) which is originally from other studies and it is unsure how sampling policies related to the fairness. Finally, Table 1 is hard to understand for me. The authors should explain the meaning of percentages (e.g., larger percentages are better?).



----------------------- REVIEW 3 ---------------------
SUBMISSION: 2376
TITLE: Counterfactual Graph Augmentation for Consumer Unfairness Mitigation in Recommender Systems
AUTHORS: Giacomo Medda, Francesco Fabbri, Mirko Marras, Ludovico Boratto and Gianni Fenu

----------- Strengths -----------
1. The paper addresses an important problem in recommender systems - consumer unfairness - and proposes an approach to mitigate it.
2. The approach leverages counterfactual explanations, which provides a unique and valuable perspective.
3. The experimental results show the effectiveness of the proposed approach in reducing disparities and achieving a better trade-off.
----------- Weaknesses -----------
1. The paper lacks a clear motivation for the proposed approach. The authors should clearly explain why counterfactual explanations are relevant and how they can be used to mitigate unfairness in recommender systems, or how they can address the limitations of existing approaches.
2. The paper could benefit from clearer explanations of the methodology, especially in the graph augmentation process and the perturbation mechanism. Some details and equations are not well-explained.
3. The paper lacks a theoretical analysis. Counterfactual is a concept from the causal theory, and causal analysis is necessary for discussing counterfactual explanations. The authors should provide more theoretical insights into the working principles of their approach.
4. The paper lacks a detailed discussion of the limitations and potential drawbacks of the proposed approach. It would be helpful to address potential challenges and limitations in the deployment of the approach in real-world scenarios.
----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
This paper proposes an approach that utilizes counterfactual explanations to mitigate unfairness in recommender systems. By augmenting the user-item interaction graph, the method aims to improve the fairness of recommendation results while maintaining recommendation utility. The proposed approach shows potential in mitigating consumer unfairness, but the paper can be improved by several aspects.
